Model Sketching by Abstraction Refinement for Lifted Model Checking (Extended Version)

In this work, we show how the use of verification and analysis techniques for model families (software product lines) with numerical features provides an interesting technique to synthesize complete models from sketches (i.e.\ partial models with holes). In particular, we present an approach for synthesizing Promela model sketches using variability-specific abstraction refinement for lifted (family-based) model checking.

==> motivate.tex <==

The \Promela\, code \SIMPLE\, in Fig.~\ref{fig:sketch1} is regarded as the ``Hello World'' example of sketching
\cite{DBLP:journals/sttt/Solar-Lezama13,DBLP:conf/pldi/Solar-LezamaRBE05}. This sketch contains one integer hole, denoted by \texttt{??}.
The synthesizer should replace the hole \texttt{??} with a constant from \Zz, such that the synthesized model
satisfies the given assertion for all possible traces in it. % to \texttt{main}.
Note that statement `\texttt{do} :: \texttt{break} :: \texttt{x++} \texttt{od}' is used
to non-deterministically initialize variable \texttt{x} of type \texttt{byte} to any integer value from
its domain $[0,255]$.

\begin{figure*}[t]
\centering
\begin{minipage}[b]{0.44\textwidth}
\centering
	$\begin{array}{ll}
\hline
 & \texttt{init} \ \{ \\
 \quad & \quad \texttt{byte} \ \texttt{x}; \, \texttt{int} \ \texttt{y}; \\
 \quad & \quad \texttt{do} :: \texttt{break} \, :: \texttt{x++} \ \texttt{od}; \\
\quad & \quad \impassign{\texttt{y}}{\texttt{??*x};} \\
\quad & \quad \texttt{assert} \, (\texttt{y} \leq \texttt{x+x}) \, \} \\
\hline
	\end{array}$
\vspace{-1mm}
\caption{The \SIMPLE\, sketch.}
\label{fig:sketch1}
\end{minipage}
\begin{minipage}[b]{0.54\textwidth}
\centering
$\begin{array}{ll}
\hline
 & \texttt{init} \ \{ \\
 \quad & \quad \texttt{byte} \ \texttt{x}; \, \texttt{int} \ \texttt{y}; \\
  \quad & \quad \texttt{do} :: \texttt{break} \, :: \texttt{x++} \ \texttt{od}; \\
\quad & \quad \texttt{\#if} :: (\texttt{A=$\Min$}) \to \impassign{\texttt{y}}{\Min\texttt{*x};}  \\
\quad & \qquad \qquad \ldots \\
\quad & \qquad \ \ \, :: (\texttt{A=$\Max$}) \to \impassign{\texttt{y}}{\Max\texttt{*x};}  \, \texttt{\#endif} \\
\quad & \quad \texttt{assert} \, (\texttt{y} \leq \texttt{x+x}) \, \} \\ \hline
\end{array}$
\vspace{-1mm}
\caption{The \SIMPLE\, model family.}
\label{fig:family1}
\end{minipage}
\vspace{-2mm}
%\caption{Motivating example \SIMPLE.} \label{fig:sketches}
\end{figure*}

\begin{figure*}
\centering
\begin{minipage}[b]{0.49\textwidth}
\centering
	$\begin{array}{ll}
\hline
 & \texttt{init} \ \{ \\
 \quad & \quad \texttt{byte} \ \texttt{x}; \, \texttt{int} \ \texttt{y}; \\
  \quad & \quad \texttt{do} :: \texttt{break} \, :: \texttt{x++} \ \texttt{od}; \\
\quad & \quad \texttt{if} :: \true \to \impassign{\texttt{y}}{\Min\texttt{*x};}  \\
\quad & \qquad \qquad \ldots \\
\quad & \qquad \ :: \true \to \impassign{\texttt{y}}{3\texttt{*x};}  \\
\quad & \qquad \qquad \ldots \\
\quad & \qquad \ :: \true \to \impassign{\texttt{y}}{\Max\texttt{*x};}  \  \texttt{fi} \\
\quad & \quad \texttt{assert} \, (\texttt{y} \leq \texttt{x+x}) \, \} \\
\hline
	\end{array}$
\vspace{-1mm}
\caption{Abstraction for $(\Min \!\leq\! \texttt{A} \!\leq\! \Max)$.}
\label{fig:abs1:1}
\end{minipage}
\begin{minipage}[b]{0.49\textwidth}
\centering
$\begin{array}{ll}
\hline
 & \texttt{init} \ \{ \\
 \quad & \quad \texttt{byte} \ \texttt{x}; \, \texttt{int} \ \texttt{y}; \\
  \quad & \quad \texttt{do} :: \texttt{break} \, :: \texttt{x++} \ \texttt{od}; \\
\quad & \quad \texttt{if} :: \true \to \impassign{\texttt{y}}{\Min\texttt{*x};}  \\
\quad & \qquad \qquad \ldots \\
\quad & \qquad \ :: \true \to \impassign{\texttt{y}}{\texttt{2*x};}  \\
\quad & \qquad \ :: \false \to \impassign{\texttt{y}}{\texttt{3*x};}  \\
\quad & \qquad \qquad \ldots \\
\quad & \qquad \  :: \false \to \impassign{\texttt{y}}{\Max\texttt{*x};}  \ \texttt{fi} \\
\quad & \quad \texttt{assert} \, (\texttt{y} \leq \texttt{x+x}) \, \} \\ \hline
\end{array}$
\vspace{-1mm}
\caption{Abstraction for $(\Min \!\leq\! \texttt{A} \!\leq\! 2)$.}
\label{fig:abs1:2}
\end{minipage}
\vspace{-2mm}
%\caption{Some abstractions of the \SIMPLE\, model family.} \label{fig:sketches}
\end{figure*}
As observed before in the literature \cite{DBLP:conf/birthday/CeskaD0JK19,DAL}, a sketch can be represented as a model
family, such that all possible sketch realizations correspond to possible variants in the model family.
For example, the \SIMPLE\, sketch can be encoded as a model family that
contains one numerical feature \texttt{A} with domain $[\Min,\Max] \subseteq \Zz$
\footnote{Note that the numerical feature \texttt{A} is represented as a global variable of type \texttt{int}, while $\Min$, $\Max$ represent
minimal and maximal representable integers. For example, we may take $\Min=0$ and $\Max=15$ for 4-bit sizes of holes.}, such that the occurrence of the hole \texttt{??} is replaced with a constant value that \texttt{A} can take.
The obtained model family \SIMPLE\, is shown in Fig.~\ref{fig:family1}, where an \texttt{\#if} directive from
the \texttt{CPP} preprocessor \cite{KastnerPhD} is used to encode multiple variants in the model family.
There is one variant for each possible configuration, i.e.\ for each possible value that \texttt{A} can take from its domain $[\Min,\Max]$ at compile-time.
Thus, there are $\Max - \Min +1$ variants that can be derived from this family.


To find a correct variant that satisfies the given assertion, we perform
an abstraction refinement procedure for lifted model checking \cite{spin15,sttt16} of the \SIMPLE\, model family.
In the first iteration, we apply the coarsest abstraction on the configuration space, thus obtaining
an abstract model with a single abstract configuration, where the \texttt{\#if} directive is
replaced with an ordinary \texttt{if} statement where all guards corresponding to various variants are enabled (i.e., set to \true).
The coarsest abstract model of the \SIMPLE\, family is shown in Fig.~\ref{fig:abs1:1}.
We can verify the obtained abstract model using the \SPIN\, model checker, which finds that the assertion fails and reports a counterexample (trace).
In this example, it reports the trace corresponding to the case when ($\texttt{A}=3$), i.e., when $\impassign{\texttt{y}}{3\texttt{*x}}$.
Hence, in the second iteration, we split the family of variants $(\Min \!\leq\! \texttt{A} \!\leq\! \Max)$ into two
sub-families $(\Min \!\leq\! \texttt{A} \!\leq\! 2)$ and $(4 \!\leq\! \texttt{A} \!\leq\! \Max)$, we construct single abstract models
for each sub-family, and repeat the verification task on each of them using \SPIN.
Fig.~\ref{fig:abs1:2} shows the abstract model corresponding to the sub-family $(\Min \!\leq\! \texttt{A} \!\leq\! 2)$.
\SPIN\, reports that this abstract model satisfies the given assertion.
Hence, we can correctly replace the hole \texttt{??}
in the original sketch with an integer value from $[\Min,2]$, so that the assertion will always be valid.
This way, we have shown that our abstraction refinement  %for lifted model checking
procedure can successfully resolve %synthesize the hole \texttt{??} in
the \SIMPLE\, sketch.


